Efficient Model-Based Multi-Agent Mean-Field Reinforcement Learning

Learning in multi-agent systems is highly challenging due to several factors including the non-stationarity introduced by agents' interactions and the combinatorial nature of their state and action spaces. In particular, we consider the Mean-Field Control (MFC) problem which assumes an asymptotically infinite population of identical agents that aim to collaboratively maximize the collective reward. In many cases, solutions of an MFC problem are good approximations for large systems, hence, efficient learning for MFC is valuable for the analogous discrete agent setting with many agents. Specifically, we focus on the case of unknown system dynamics where the goal is to simultaneously optimize for the rewards and learn from experience. We propose an efficient model-based reinforcement learning algorithm, $M^3-UCRL$, that runs in episodes, balances between exploration and exploitation during policy learning, and provably solves this problem. Our main theoretical contributions are the first general regret bounds for model-based reinforcement learning for MFC, obtained via a novel mean-field type analysis. To learn the system's dynamics, $M^3-UCRL$ can be instantiated with various statistical models, e.g., neural networks or Gaussian Processes. Moreover, we provide a practical parametrization of the core optimization problem that facilitates gradient-based optimization techniques when combined with differentiable dynamics approximation methods such as neural networks.

==> TMLR_ArXiv Submission_arXiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> TMLR_ArXiv Submission_arXiv/sections/1-introduction.tex <==
\vspace{-1ex}
\section{Introduction}
Multi-Agent Reinforcement Learning (MARL) extends the scope of reinforcement learning (RL) to multiple agents acting in a shared system. It is receiving considerable attention given a great number of real-world applications including autonomous driving \citep{shalev2016safe}, finance \citep{lee2002stock,lee2007multiagent,Lehalle2019ACorrelations}, social science \citep{castelfranchi2001theory,leibo2017multi}, swarm motion \citep{Almulla2017TwoGames}, e-sports \citep{vinyals2019grandmaster, pachocki2018openai}, and traffic routing \citep{eltantawy2013Multiagent}, to name a few.
Despite the recent popularity, analyzing agents' performance in these systems remains a particularly challenging task for several reasons including non-stationarity, scalability, competing learning goals, and varying information availability of agents. In this work, we target the challenges of \emph{non-stationarity} and \emph{scalability}. From the perspective of an individual agent, the dynamics of the system are non-stationary, since other agents update their behaviour, which alters over time how the environment reacts to certain actions of the agent. Multi-agent systems also suffer from a \emph{combinatorial nature} due to the exponential growth of the state and action space as the number of agents in the system increases. 
\looseness=-1

\looseness=-1
To tackle the previous challenges, {\em Mean-Field Control} (MFC) exploits the insight that many relevant MARL problems involve a large number of {\em very similar} agents that are coordinated via a centralized controller. As a motivating application, consider a ride-hailing service in which a central dispatcher coordinates the routes of many drivers around the city. MFC considers the limiting regime of controlling {\em infinitely many identical collaborative} agents, and utilizes the notion of mean-field approximation from statistical physics \citep{weiss1907hypothese} to model their interactions. Specifically, instead of focusing on the individual agents and their interactions, the state of the system is described via the agents' state distribution and the dynamics and rewards are formulated accordingly. Despite the introduced approximations, the solution to the MFC problem often remains adequate for the finite agent equivalent \citep{lacker2017limit}.
\looseness=-1

The focus of this work is on learning the optimal policies in MFC when the underlying dynamics are {\em unknown}. In complex domains such as fleets of autonomous vehicles or robot swarms, this is often the case, and the models consequently need to be learnt from data, giving rise to a well-known exploration--exploitation dilemma.
In this paper, we propose the \emph{Model-Based Multi-Agent Mean-Field Upper-Confidence RL} algorithm (\mfhucrl) that is provably efficient and can effectively trade-off between exploration and exploitation during policy learning.
Similarly to other Model-Based Reinforcement Learning (MBRL) algorithms, \mfhucrl collects data about the unknown dynamics online (i.e., by proposing and executing a policy in the true system) and estimates the possible dynamics the system might follow. To optimize the agent's actions, it simulates the unknown system by using the estimated dynamics. \citet{chua2018deep} has shown that MBRL can solve challenging single-agent RL problems with low sample complexity. We transfer this property to multi-agent problems and show that \mfhucrl can efficiently solve the MFC problem with unknown dynamics.
\looseness=-1



==> TMLR_ArXiv Submission_arXiv/sections/2-related_work.tex <==
\textbf{Related work.} Our \mfhucrl extends the class of Model-Based Reinforcement Learning (MBRL) algorithms that rely on the \emph{optimism-in-the-face-of-uncertainty} principle. 
Algorithms based on this approach achieve optimal regret for tabular MDPs \citep{brafman2002r, auer2009near, efroni2019tight, domingues2020regret}, while in the continuous setting,
\cite{Abbasi-Yadkori2011RegretSystems} and \cite{jin2020provably} show $\Tilde{\mathcal{O}}(\sqrt{T})$ regret bounds for LQR and linear MDPs, respectively. The recently designed episodic model-based algorithms \citep{chowdhury2019online, kakade2020information, curi2020efficient, Sessa2022EfficientComputation} achieve similar regret in the kernelized setting.
\citet{Sessa2022EfficientComputation} consider the general multi-agent setting, and prove a regret bound with $\mathcal{O}(N^{H/2})$ dependence on the number $N$ of agents. In comparison, \mfhucrl assumes an asymptotically large population of identical agents. Crucially, as we will show, its performance does {\em not} depend on the number of agents, making it more suitable for large systems.
\looseness=-1



{\em Multi-Agent Reinforcement Learning (MARL)} has seen tremendous progress in recent years as many real-world applications involve interactions among a number of agents.
\cite{Busoniu2008ALearning} provide an overview of classical and early MARL results. Several other MARL surveys focus on: non-stationarity induced by the agent interactions \citep{Hernandez-Leal2017ANon-Stationarity}, deep MARL \citep{Hernandez-Leal2019ALearning, Nguyen2020DeepApplications}, theoretical foundations in Markov/stochastic/extensive-form games \citep{Zhang2019Multi-AgentAlgorithms} and cooperative MARL \citep{OroojlooyJadid2019ALearning}.
Recently, \cite{Zhang2019Multi-AgentAlgorithms} and \cite{Nguyen2020DeepApplications} recognize the lack of practical model-based MARL algorithms (with an early exception of the R-Max algorithm proposed by \cite{brafman2000near, brafman2002r} for two-player zero-sum Markov Games). We fill this gap by designing a practical model-based algorithm that considers a large population of agents, and that is compatible with deep models.\looseness=-1





Modeling interaction via the mean-field approach in MARL has recently gained popularity due to the introduction of Mean-Field Games (MFG) \citep{lasry2006jeux1,lasry2006jeux2, huang2006large, huang2007large}. MFG consider the limiting regime of a competitive game among identical agents with the objective of reaching a Nash Equilibrium. Various works \citep{Yin2010LearningGames, Yin2014LearningGames, Cardaliaguet2017LearningPlay, gueant2011mean, bensoussan2013mean, carmona2013probabilistic, carmona2018probabilistic, gomes2014mean} mainly consider solving MFGs in continuous-time, while some very recent ones \citep{Yang2017LearningBehavior, yang2018mean, Fu2019Actor-CriticGames, Guo2019LearningGames, Guo2020AGames, elie_convergence_2019, agarwal_reinforcement_2019} analyze the problem from the discrete-time RL perspective. The progress of the field has been recently summarized by \citet{LauriereLearningSurvey}.\looseness=-1%

At the same time, cooperative discrete-time {\em Mean-Field Control}, the main focus of this paper, has received significantly less attention. \citet{gast2012mean, Motte2019Mean-fieldControls, Gu2019DynamicMFCs,  Gu2021Mean-FieldAnalysis} and \citet{Bauerle2021MeanProcesses} consider planning with known dynamics.
In the learning setting, \citet{wang2020breaking, carmona2019model, Gu2021Mean-FieldAnalysis, Angiuli2022UnifiedProblems, Angiuli2021ReinforcementEconomics} extend the Q-Learning algorithm and show convergence for specific variants of MFC focusing on discrete state and action spaces.
The mean-field extension of the linear-quadratic problem has been studied by \citet{Carmona2019Linear-QuadraticMethods, Wang2021GlobalTime, Carmona2021Linear-quadraticOptimization} with policy optimisation methods.
\citet{subramanian_reinforcement_2019} also proposes a policy-gradient based algorithm that solves Mean-Field Games and Control problems locally.
Additionally, \citet{Chen2021PessimismRL, Li2021PermutationApproach, wang2020breaking} consider the approximation error between the Mean-Field and the related Multi-Agent Reinforcement Learning problems.
These previous model-free methods are either sample inefficient, assume access to a simulator or consider finite state and action spaces. On the contrary, our algorithm is model-based, sample-efficient, works for continuous spaces and learns the policy online by performing exploration on a real system.\looseness=-1


\textbf{Main contributions.} We design a novel \emph{Model-based Multi-agent Mean-field Upper Confidence} RL (\mfhucrl) algorithm for the centralized control problem of a large population of collaborative agents. \mfhucrl is practical, performs exploration on a real system (requires no simulator and efficient in terms of samples), and is compatible with neural network policy learning. Our main contributions are the general theoretical regret bounds obtained via a novel mean-field-based analysis, that we also specialize to Gaussian Process models. In the main step of our theoretical analysis, we bound the distance between the mean-field distributions under the true and the approximated dynamics via the model's total estimated uncertainty.
Finally, we pose the exploration via entropy maximization problem used in a recent MFG survey \citep{LauriereLearningSurvey} in the continuous state and action domain and demonstrate the performance of our algorithm in it. Our results show that \mfhucrl is capable of finding close-to-optimal policies within a few episodes, in contrast to model-free algorithms that require at least six orders of magnitude more samples.


==> TMLR_ArXiv Submission_arXiv/sections/3.2-problem_statement.tex <==
\vspace{-1ex}
\section{Problem Statement}
\label{section:ProblemStatement}

We consider the episodic Mean-Field Control (MFC) problem with time-horizon $H$, compact state space $\stateSpace{} \subseteq \mathbb{R}^p$ and compact action space $\actionSpace{} \subseteq \mathbb{R}^q$ that are common for all the agents in the system. We index episodes with the variable $t$ and use $T$ to denote the number of episodes passed.
In standard $N$-agent settings, the system's state in episode $t$ at time $h \in \lbrace 0, \dots, H-1 \rbrace$ is described with individual agents' states $(\state{t,h}{(1)}, \dots, \state{t,h}{(N)}) \in \stateSpace{N}$ which grows exponentially in the number of agents $N$ and represents a common issue in scaling MARL algorithms. In MFCs, we assume that all agents are \emph{identical} and the population is \emph{asymptotically infinite}, i.e., $N\to\infty$, therefore, the agents' states can be described by the \emph{mean-field distribution}:
\vspace{-5pt}
\begin{equation*}
        \stateDist{t,h}(s) = \lim_{N \to \infty} \frac{1}{N} \sum_{i=1}^N \mathbb{I}_{ \lbrace \state{t,h}{(i)} = s \rbrace },
        \vspace{-5pt}
\end{equation*}
where $\stateDist{t,h}$ belongs to the space of probability measures $\stateDistSpace$ over $\stateSpace{}$. Due to the assumption of \emph{identical} agents in MFC, we can focus on a \emph{representative agent} from the population that interacts with the distribution of agents instead of individual agents and interactions.

\textbf{System Dynamics.} Before every episode $t$, the representative agent selects a policy profile $\policyProfile{t}{} = (\policy{t,0}{}, \dots, \policy{t,H-1}{})$ where the $H$ individual policies $\policy{t,h}{}: \stateSpace{} \times \stateDistSpace \rightarrow \actionSpace{}$ 
are chosen from a set of admissible policies $\admissiblePolicies{}$ (e.g., we parametrize our polices via neural networks; see below). At every time $h$, the representative agent selects an action $ \action{t,h}{} = \policy{t,h}{} (\state{t,h}{}, \stateDist{t,h})$. 
The environment then returns reward $r^{}(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h})$, and the agent observes its new state $\state{t,h+1}{}$ and the mean-field distribution $\stateDist{t,h+1}$.
\looseness=-1

In MFCs, the system's dynamics are typically given by a McKean-Vlasov type of stochastic processes and depend on the agent's state, action and the mean-field distribution:\looseness=-1
\vspace{-2pt}
\begin{equation}
    \state{t,h+1}{} = f(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}) +   \noise{t,h}{},
    \label{eq:transitionDynamics}
    \vspace{-1pt}
\end{equation}
where $\noise{t,h}{}$ is an \emph{i.i.d.}~additive noise vector. This is in contrast to the standard single-agent model-based RL (cf. \cite{chowdhury2019online,curi2020efficient,kakade2020information}), where the dynamics only depend on agent's action and state. Crucially, since the focus of this work is on {\em learning} in MFC, we assume that the true dynamics are \emph{unknown}, and the goal is to explore the space and learn about $f$ over a number of episodes.
\footnote{
    We expect our results to easily extend and account for unknown rewards by using the same modeling assumptions for the reward function (e.g., as in  \cite{chowdhury2019online}).\looseness=-1
}
To do so, the representative agent relies on the collected random observations, $\mathcal{D}_{t} = \lbrace((\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}), \state{t,h+1}{})\rbrace_{h=0}^{H-1}$, which come from the interaction with the true system (i.e., from policy rollouts) during episode $t$.

Finally, after every episode, we assume that the whole system is reset and the agent's initial state $\state{0}{}$ is drawn from a known initial distribution $\stateDist{0}$, i.e., $\state{0}{} \sim \stateDist{0}$, that remains the same in every episode. 

\textbf{Mean-field Flow.} Since, in MFC, all agents are identical, interact in a common environment, and follow the \emph{same policy} $\policyProfile{t}{}=(\policy{t,0}{}, \dots, \policy{t,H-1}{})$, the subsequent mean-field distributions satisfy the following mean-field flow property as shown by \cite{Gu2019DynamicMFCs}:\looseness=-1
\begin{lemma}
    \label{lemma:MFDistributionTransition}
    For a given initial distribution $\stateDist{0}$, dynamics $f$ and policy $\policyProfile{}{} = (\policy{0}{}, \dots, \policy{h-1}{})$, the mean-field distribution trajectory $\lbrace\stateDist{h}\rbrace_{h=0}^{H-1}$, follows
    \begin{equation}
        \stateDist{h+1}(ds') =
            \int_{s \in \stateSpace{}} \stateDist{h} (ds) \mathbb{P}[ \state{h+1}{} \in ds'],
    \label{eq:flowdynamics}
    \end{equation}
    where $\stateDist{h} \in \stateDistSpace$ for all $h \geq 0$, $\action{h}{} = \policy{h}{} (\state{h}{}, \stateDist{h})$, $\state{h+1}{}$ is given by \cref{eq:transitionDynamics}, and $\stateDist{h} (ds) = \mathbb{P}[\state{h}{} \in ds]$ under $\policyProfile{}{}$.
\end{lemma}

We provide the proof in \cref{appendix:measure_formulation}. 
To shorten the notation, we use $\Phi (\stateDist{t,h}, \policy{t,h}{}, f)$ to denote the mean-field transition function from \cref{eq:flowdynamics}, i.e., we have 
$\stateDist{t,h+1}{} = \Phi (\stateDist{t,h}, \policy{t,h}{}, f)$. 
The lemma shows that the next mean-field distribution explicitly depends on the unknown $f$ (since $\state{t,h+1}{} = f(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}) + \noise{t,h}{}$), policy played by the agents $\policy{t,h}{}$, and previous state distribution $\stateDist{t,h}$.\looseness=-1

\textbf{Performance metric.} Given a policy profile $\policyProfile{}{} = (\policy{1}{}, \dots, \policy{H-1}{})$, the performance of the representative agent is measured via the expected cumulative reward:\looseness=-1
\begin{subequations}
    \label{eq:expectedCumulativeReward}
    \begin{align}
        \mathbb{J}(\policyProfile{}{}) &= \mathbb{E} \bigg[
                \sum_{h=0}^{H-1} r(\state{h}{}, \action{h}{}, \stateDist{h})
            \bigg]\\
        \text{s.t.} \quad \action{h}{} &= \policy{h}{}(\state{h}{}, \stateDist{h}), \\
        \state{h+1}{} &= f(\state{h}{}, \action{h}{}, \stateDist{h}) + \noise{h}{}, \\
        \stateDist{h+1} &= \Phi (\stateDist{h}, \policy{h}{}, f),
    \end{align}
\end{subequations}
where the expectation is taken over the noise in the transitions and initial distribution $\state{0}{} \sim \stateDist{0}$. By considering the representative agent's perspective, the goal is to discover a \emph{socially} optimal policy $\policyProfile{}{*}$ that maximizes the expected total reward, i.e.,
\looseness=-1
\begin{equation}
    \policyProfile{}{*}\in\arg\max_{\policyProfile{}{}} \;\mathbb{J}(\policyProfile{}{})
    \label{eq:MFCOptimizationObjective}
\end{equation}
In our theoretical analysis, we make the following assumptions regarding the system's true dynamics, reward function and the set of admissible policies. We use $\jointState{}{}, \jointState{}{}' \in \jointStateSpace{} = \stateSpace{} \times \actionSpace{} \times \stateDistSpace$ to denote $(\state{}{}, \action{}{}, \stateDist{})$ and $(\state{}{}', \action{}{}', \stateDist{}')$, respectively, and we make use of the Wasserstein-1 metric:
$
    W_1(\stateDist{}, \stateDist{}') = \inf_{\nu}
            \int_{\stateSpace{} \times \stateSpace{}} \norm{x - y}_{2} d\nu(x, y),
$
where $\nu$ is any probability measure on $\stateSpace{} \times \stateSpace{}$ with marginals $\stateDist{}$ and $\stateDist{}'$ (see \cref{section:appendix_wasserstein} for useful properties of $W_1(\stateDist{}, \stateDist{}')$ that are used in our analysis).
    
\begin{assumption}
    \label{assumption:LipschitzDynamics}
    The transition function $f$ is $L_f$--Lipschitz-continuous, i.e., $\norm{f(\jointState{}{}) - f(\jointState{}{})}_2 \leq L_f d(\jointState{}{},\jointState{}{}')$
    where $d(\jointState{}{},\jointState{}{}'):= \norm{\state{}{} - \state{}{}'}_2 + \norm{\action{}{} - \action{}{}'}_2 + W_1 (\stateDist{}, \stateDist{}')$ and $\noise{t,h}{}$ are \emph{i.i.d.} additive $\sigma$-sub-Gaussian noise vectors for all $t \geq 1$ and $h \in \lbrace 0,\dots, H-1\rbrace$.
\end{assumption}


\begin{assumption}
    \label{assumption:LipschitzPolicyAndReward}
    The set of admissible policies $\admissiblePolicies{}$ consists of $L_{\policy{}{}}$--Lipschitz-continuous policies such that for any $\policy{}{} \in \admissiblePolicies{}\mathrm{:}
    \norm{ \policy{}{}(\state{}{}, \stateDist{}) - \pi(\state{}{}', \stateDist{}') }_2 \leq L_{\policy{}{}} (\norm{\state{}{} - \state{}{}'}_2 + W_1(\stateDist{}, \stateDist{}')),$ and the reward function is $L_{r}$--Lipschitz-continuous, i.e., $|r(\jointState{}{}) - r(\jointState{}{}')|\leq L_r d(\jointState{}{},\jointState{}{}').$
\end{assumption}

Regularity assumptions like these are standard in the single-agent model-based reinforcement learning literature \citep{jaksch2010near, curi2020efficient, chowdhury2019online, Sessa2022EfficientComputation} and mild since, in practice, the policy and reward function classes are typically chosen to satisfy the previous smoothness assumptions. In our experiments (see \cref{section:experiments}), we parametrize our policies with Neural Networks with Lipschitz continuous activations (e.g., $\operatorname{tanh}$, $\operatorname{ReLU}$ and $\operatorname{linear}$). We note that the Lipschitzness of such policies then follows from that of the activations when the network’s weights are bounded (in practice, this can be done by directly bounding them or via regularization).

\begin{remark}
    The episodic Mean-Field Control problem relates closely to the finite-horizon case of the evolutive Mean-Field Game problem described in \citet{LauriereLearningSurvey}. Both settings consider mean-field distributions evolving over time depending on the agents' policies, however, the MFC problem focuses on collaborative agents while agents in the evolutive MFG are competitive. This distinction leads to different solution concepts of the problems; social welfare in MFC and Nash Equilibrium in MFG.
\end{remark}
\looseness=-1








==> TMLR_ArXiv Submission_arXiv/sections/4-algorithm.tex <==
\vspace{-1ex}
\section{The \mfhucrl Algorithm}
    \label{section:algorithm}
    In this section, we tackle the Mean-Field Control Problem with unknown dynamics from \cref{eq:MFCOptimizationObjective} by relying on a \emph{model-based} learning scheme. Our \emph{Model-based Multi-agent Mean-field Upper Confidence} RL (\mfhucrl) algorithm uses a statistical model to estimate the system's dynamics and %
    to effectively trade-off between exploration and exploitation during policy learning. Before stating our algorithm, we consider the main properties of the considered dynamics models.
    
          
          
    
    \textbf{Statistical Model.} Our representative agent learns about the unknown dynamics from the data collected during the interactions with the environment, i.e., the policy rollouts. In particular, we take a model-based perspective (see \cref{alg:M^3_outline}), where the agent models the unknown dynamics and sequentially, after every episode $t$, updates and improves its model estimates based on the previous transition observations, i.e., $\mathcal{D}_{1} \cup \dots \cup \mathcal{D}_{t}$ where $\mathcal{D}_{t} = \lbrace((\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}), \state{t,h+1}{})\rbrace_{h=0}^{H-1}$ is the set of state transition observations in episode $t$.
    To reason about plausible models at every episode $t$, the representative agent can take a frequentist or Bayesian perspective. In the first case, it estimates the mean $\modelMean{t}: \jointStateSpace{} \to \stateSpace{}$ and confidence $\modelStdMatrix{t}: \jointStateSpace{}{} \to \mathbb{R}^{p \times p}$ functions.
    In the second case, the agent estimates the posterior distribution over dynamical models $p(\tilde{f}|\mathcal{D}_{t})$, that leads to $\modelMean{t}(z) = \mathbb{E}_{\tilde{f} \sim p(\tilde{f}|\mathcal{D}_{t})}[\tilde{f}(z)]$, and $\modelStdMatrix{t}^{2}(z) = \text{Var}[\tilde{f}(z)]$.
    We denote $\modelStd{t}(\cdot) = \diag (\modelStdMatrix{t} (\cdot))$ and make the following assumptions regarding the considered statistical model irrespective of the taken perspective:
    \looseness=-1
    \begin{assumption}[Calibrated model]
        \label{assumption:WellCalibratedModel}
        The statistical model is calibrated w.r.t. $f$, i.e., there is a known non-decreasing sequence of confidence parameters $\lbrace \modelScale{t} \rbrace_{t\geq 0}$, each $\modelScale{t} \in \mathbb{R}_{> 0}$ and depending on $\delta$, such that with probability at least $1-\delta$, it holds jointly for all $t$ and $\jointState{}{} \in \jointStateSpace{}$ that $|f(\jointState{}{}) - \modelMean{t} (\jointState{}{}) | \leq \modelScale{t} \modelStd{t} (\jointState{}{})$ elementwise.
        \looseness=-1
    \end{assumption}
    
    \begin{assumption}
        \label{assumption:LipschitzModelStd}
        The function $\modelStd{t}(\cdot)$ is $L_{\modelStd{}}$-Lipschitz-continuous for all $t \geq 1$.%
    \end{assumption}
    The calibrated model assumption (or its equivalents) is standard in online model-based learning \citep{srinivas2010gaussian, chowdhury2017onKernelized, chowdhury2019online, curi2020efficient, Sessa2022EfficientComputation}. It states that the agent can build high probability confidence bounds around the unknown dynamics at the beginning of every episode. As more observations become available, we expect the \emph{epistemic} uncertainty of the model (that arises due to the lack of data and is encoded in $\modelStd{}(\cdot)$) to shrink, and consequently allow the representative agent to make better decisions as it becomes more confident about the true dynamics. %
    Our theoretical results obtained in \cref{section:theoretical_results} hold for general model classes as long as \cref{assumption:WellCalibratedModel} and \cref{assumption:LipschitzModelStd} are satisfied. Below and in \cref{section:theoretical_results}, we provide concrete conditions (about $f$) and models for which this assumption provably holds.
    \looseness=-1
    
          
          
    
    
    \textbf{Algorithm.} At the beginning of episode $t$, the representative agent constructs the confidence set of dynamics functions, denoted by $\mathcal{F}_{t-1}$, satisfying the elementwise confidence interval in \cref{assumption:WellCalibratedModel} with $\modelMean{t-1}(\cdot)$ and $\modelStd{t-1}(\cdot)$ estimated based on the observations up until the end of the previous episode $t-1$, i.e.,\looseness=-1
    \begin{equation*}
        \mathcal{F}_{t-1} = 
        \Big\lbrace \approxDynamics{}: |\approxDynamics{}(z) - \modelMean{t-1}(z)| \leq \beta_{t-1} \modelStd{t-1}(z) \text{ elementwise and }\forall z \in \jointStateSpace{}  \Big\rbrace.
    \end{equation*}
    Then, the agent selects the optimistic policy $\policyProfile{t}{}$ which achieves the highest possible cumulative reward over the set of admissible policies, $\Pi$, and plausible system dynamics $\mathcal{F}_{t-1}$.
    In particular, the representative agent solves the following problem:
    \looseness=-1
    \begin{subequations} \label{eq:UCBOptimization}
        \begin{align} \label{eq:UCBObjective}
            \policyProfile{t}{} &= \argmax_{\policyProfile{}{} \in \Pi} \max_{\approxDynamics{} \in \mathcal{F}_{t-1}} \mathbb{E}
            \left[
                \sum_{h=0}^{H-1} r(\OptState{t,h}, \OptAction{t,h}, \OptStateDist{t,h})
            \right] \\
            &\text{s.t.}\quad \OptAction{t,h} = \policy{t,h}{}(\OptState{t,h}, \OptStateDist{t,h}), \\
            \label{eq:OptimizationStateTransition}
            &\quad \; \OptState{t,h+1} = \approxDynamics{}(\OptState{t,h}, \OptAction{t,h}, \OptStateDist{t,h}) + \OptNoise{t,h}, \\
            \label{eq:OptimizationStateDistributionTransition}
            &\quad \;\OptStateDist{t,h+1} = \Phi(\OptStateDist{t,h}, \policy{t,h}{}, \approxDynamics{}),
        \end{align}
    \end{subequations}
    where the expectation in \cref{eq:UCBObjective} is taken w.r.t.~the initial state distribution $\stateDist{0}$ and noise in transitions.
    \looseness=-1
    
    The policy $\policyProfile{t}{}$ found by solving the previous problem is then used in the true multi-agent system (e.g., used by every driver in a ride-hailing service) for one episode. It induces the observed mean-field flow, and aims to improve the total collective reward. After the episode ends, the representative agent augments its observed data, i.e., $\mathcal{D}_{1:t} =  \mathcal{D}_{1:t-1}  \cup \mathcal{D}_{t}$, and improves its model estimates $\modelMean{t}(\cdot)$ and $\modelStd{t}(\cdot)$. The algorithm is summarized in \cref{alg:M^3_outline}. Since solving \cref{eq:UCBOptimization} is a challenging task even for known dynamics and the focus of this work is on the statistical complexity of learning in MFC (similarly to \citet{kakade2020information, chowdhury2019online, curi2020efficient, Sessa2022EfficientComputation}), we assume that we can solve \cref{eq:UCBOptimization} for a given $\mathcal{F}_{t-1}$ and $\Pi$. We propose a practical implementation below with details on solving \cref{eq:UCBOptimization}.

    \begin{algorithm}[t]
    \caption{Model-based RL for Mean-field Control}
    \label{alg:M^3_outline}
    \begin{algorithmic}
        \State{\bfseries Input:} Calibrated dynamical model, reward function $r^{}(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h})$, horizon $H$, initial state $\state{1,0}{} \sim \stateDist{0}{}$\looseness=-1
        \For{$t=1,2,\dots$}
            \State \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{%
                Use \mfhucrl to select policy profile $\policyProfile{t}{}=(\policy{t,0}{}, \dots, \policy{t,h-1}{})$ by using the current dynamics model and reward function, i.e., solve \cref{eq:UCBOptimization}%
            }
        \For {$h=0, \dots, H-1$}
            \State 
            $
                \action{t,h}{} = \pi_{t,h}(\state{t,h}{}, \stateDist{t,h}), 
            $
            \State 
            $
                \state{t,h+1}{} = f(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}) + \noise{t,h}{}
            $
            \State
                $\stateDist{t,h+1}{} = \Phi (\stateDist{t,h}, \policy{t,h}{}, f)$
          \EndFor
          \State Update agent's statistical model with new observations $\lbrace(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}), \state{t,h+1}{}\rbrace_{h=0}^{H-1}$
          \State Reset the system to $\stateDist{t+1, 0} \leftarrow \stateDist{0}$ and $\state{t+1,0}{} \sim \stateDist{t+1,0}$
          \EndFor
        \end{algorithmic}
    \end{algorithm}
    \vspace{-5pt}
    
    The algorithm implements the \emph{upper-confidence bound} principle,  since  the  system's true dynamics $f$ belong to the confidence set $\mathcal{F}_{t-1}$ with high-probability (by \cref{assumption:WellCalibratedModel}). Consequently,  the  reward  achieved  by $\policyProfile{t}{}$ under the best possible dynamics $\approxDynamics{}$  upper bounds the performance of $\policyProfile{t}{}$ under the true dynamics $f$.\looseness=-1
    
    
    \textbf{Practical Implementation.}
    In general, optimizing over the set $\mathcal{F}_{t-1}$ is not tractable. However, a practical problem reformulation has been designed \citep{moldovan2015optimism, curi2020efficient} for single-agent problems, which defines an auxiliary policy to select the dynamics function $\approxDynamics{} \in \mathcal{F}_{t-1}$. We generalize this approach to the MFC setting to implement
    \mfhucrl for our experiments (see \cref{appendix:HallucinatedControl} for details).\looseness=-1
    
    \mfhucrl can be combined with any statistical model that satisfies \cref{assumption:WellCalibratedModel}. For example, under mild assumptions on the unknown dynamics, Gaussian Processes (GP) models \citep{rasmussen2003gaussian} can be provably calibrated under some regularity assumptions on the dynamics \citep{srinivas2010gaussian, Abbasi-Yadkori2011RegretSystems}. Neural Network (NN) models  \citep{anthony2009neural} such as Probabilistic and Deterministic Ensembles \citep{lakshminarayanan2016simple, chua2018deep} are more scalable, and even though they are not calibrated by default, their empirical recalibration is possible \citep{kuleshov2018accurate}. Finally, using such differentiable dynamics models and parameterizing $\policyProfile{t}{}(\cdot)$ and the auxiliary policy selecting $\approxDynamics{}$ via separate neural networks, allows for optimizing \cref{eq:UCBOptimization} by using gradient-based approaches (see \cref{appendix:experimentImplementation}).
    \looseness=-1 
    

    
\begin{remark}
    \mfhucrl uses an optimistic upper-confidence bound strategy similarly to single-agent model-based upper-confidence algorithms \citep{chowdhury2019online, kakade2020information, curi2020efficient, Sessa2022EfficientComputation}, however, it addresses several important differences:
    (i) dynamics and rewards explicitly depend on the states of all agents through the mean-field distribution;
    (ii) each agent's action depends on the mean-field distribution and the evolution of the mean-field trajectory is induced by the collection of actions taken by the agents;
    (iii) crucially, \mfhucrl employs the principle that each agent in the system executes the same policy selected by the representative agent;
    Moreover, we note that single-agent MBRL algorithms are inherently unsuitable for solving the Mean Field Control problem.
    \looseness=-1
\end{remark}

==> TMLR_ArXiv Submission_arXiv/sections/5-results.tex <==
\vspace{-1ex}
\section{Theoretical Analysis}
    \label{section:theoretical_results}
    We analyze our approach using the standard notion of {\em cumulative regret}. It measures the difference in the cumulative expected reward between the socially optimal policy $\policyProfile{}{*}$ (from 
    \cref{eq:MFCOptimizationObjective}) and the individual policies selected by \mfhucrl in every episode: $R_{T} = \sum_{t=1}^{T} (\mathbb{J}(\policyProfile{}{*}) - \mathbb{J}(\policyProfile{t}{}))$. We also use $r_t$ to denote the regret incurred during episode $t$, i.e., 
    $r_t := \mathbb{J}(\policyProfile{}{*}) - \mathbb{J}(\policyProfile{t}{})$.
    We aim to show that \mfhucrl achieves {\em sublinear} cumulative regret, i.e., $\lim_{T \to \infty} \frac{1}{T} R_{T} = 0$. 
    This implies that as the number of episodes increases, the performance of the selected policies converges to that of the optimal policy: $\mathbb{J}(\policyProfile{t}{}) \to \mathbb{J}(\policyProfile{}{*})$. We defer all the proofs from this section to \cref{appendix:RegretBoundProof} and only highlight the main contributions of our work.\looseness=-1
    
    
    In general, the speed of convergence of \mfhucrl will depend on the difficulty of estimating $f$. For more complex functions, we expect our models to require more observations to achieve close approximation of the underlying dynamics. Consequently, we use the following model-based complexity measure to quantify this aspect of the learning problem:
    \looseness=-1
    \begin{equation}
    \vspace{-1mm}
        \label{eq:complexityMeasure}
        I_{T} = \max_{\tilde{D}_{1}, \dots, \tilde{D}_{T}} \; \sum_{t=1}^{T} \sum_{\jointState{}{} \in \tilde{D}_{1} \cup \cdots \cup \tilde{D}_{t} } \norm{\modelStd{t-1}(\jointState{}{})}_{2}^{2},
    \vspace{-1mm}
    \end{equation} where $\tilde{D}_{t}$ is a set of possible observations in an episode for each $t=1,\dots,T$, and $\modelStd{t-1}(\cdot)$ is the confidence estimate of the selected statistical model computed based on $\tilde{D}_{1} \cup \cdots \cup \tilde{D}_{t-1}$. We note that the analogous notion of model complexity has been recently used in single agent model-based RL \citep{chowdhury2019online,curi2020efficient} and the multi-agent setting \citep{Sessa2022EfficientComputation}. Intuitively, $I_{T}$ measures the chosen model's total confidence in estimating the dynamics over $T$ episodes in the worst-case, i.e., when the sets of observations $\tilde{D}_{1}, \dots, \tilde{D}_{T}$ are the least informative about the unknown dynamics $f$. For statistical models that fail to learn and generalize, $I_{T}$ may grow linearly with $T$. %
On the other hand, for models that learn from a "small" number of samples, we expect $\modelStd{t-1}(\cdot)$ to shrink fast.
   
    
    \textbf{General Model-based Regret Bound.} The following theorem bounds the cumulative regret after $T$ episodes in terms of the model complexity measure $I_{T}$ defined in \cref{eq:complexityMeasure}.
    \begin{theorem}
    \label{thm:main}
    Under \Crefrange{assumption:LipschitzDynamics}{assumption:LipschitzModelStd}, let $\overline{L}_{T-1} = 1 + 2 (1 + L_{\policy{}{}})\left[
         L_f + 2 \modelScale{T-1} L_{\modelStd{}}
        \right]$,
    and let $\stateDist{t,h}{} \in \stateDistSpace{}$ for all $t,h>0$. Then for all $T \geq 1$ and fixed constant $H>0$, with probability at least $1-\delta$, the regret of \mfhucrl is at most:
    \looseness=-1
    \begin{equation}
    \begin{split}
        R_T = \mathcal{O} \Big(
        \modelScale{T} L_{r} (1+L_{\policy{}{}}) \overline{L}_{T-1}^{H-1} \sqrt{H^{3} T I_{T}}
        \Big).
    \end{split} \nonumber
    \end{equation}
    \end{theorem}
    The obtained regret bound explicitly depends on constant factors that describe the environment such as the episode horizon $H$ and the Lipschitz constants. The dependence on the size of the problem, i.e., $p$ and $q$, is implicit in $\beta_T$ and $I_T$ and specific to the statistical model used in the algorithm. We provide more explicit dependencies for Gaussian Processes below and in \cref{appendix:GaussianProcess}. We also note that $\beta_T$ is a function of $\delta$ (see \cref{assumption:WellCalibratedModel}). When polices are selected according to \cref{eq:UCBOptimization} at every episode, our result implies that the obtained performance $\mathbb{J}(\policyProfile{t}{})$
    eventually converges to the optimal one $\mathbb{J}(\policyProfile{}{*})$ if the joint dependence on the model-dependent quantities $I_{T}$ and $\modelScale{T}$ scales as $\mathcal{O}(\sqrt{T})$.\looseness=-1

    In comparison to other model-based algorithms, both \mfhucrl and H-UCRL \citep{curi2020efficient} achieve $\mathcal{O}(\sqrt{H^3TI_T})$ regret while H-MARL \citep{Sessa2022EfficientComputation} achieves $\mathcal{O}(N^{H/2} \sqrt{H^3T I_T})$. The additional factor of $\mathcal{O}(N^{H/2})$ comes from the fact that H-MARL considers separate agents with individual action spaces while \mfhucrl optimises for a representative agent instead.
    In terms of tightness of our results, we  expect that the dependency on $\mathcal{O}(\sqrt{T I_T})$ in the regret bound is unavoidable. \citet{Scarlett2017LowerOptimization} showed that this is a lower bound for the kernelized bandit problem for specific kernels and using a Gaussian Process.
    This result relates to the special case of MFC when $H=1$ and using Gaussian Process statistical model to estimate the transition dynamics. The dependency on $H^3$, however, could be improved under more restrictive assumptions.
    
    In our theoretical analysis, %
    we address non-trivial challenges that arise from considering an infinite number of agents. In particular, we first translate the Mean Field Control to a non-standard MDP with the distributional state space $\stateDistSpace{}$ and action space $\admissiblePolicies{}$ of all admissible policies (for details, see \cref{appendix:measure_formulation}). This enables us to use the upper-confidence bound principle with the assumption of well-calibrated models to show the following bound on the episodic regret:
    \begin{equation*}
        r_{t} \leq 2 L_{r}(1 + L_{\policy{}{}}) \sum_{h=1}^{H-1} W_{1} (\stateDist{t,h}{}, \OptStateDist{t,h}{}),
    \end{equation*}
    where $\stateDist{t,h}{}$ and $\OptStateDist{t,h}{}$ are the mean-field distributions when the policy $\policyProfile{t}{}$ is deployed in (i) the true multi-agent system and (ii) the system with dynamics given by the transition function $\tilde{f}_{t}$ selected by the oracle corresponding to $\policyProfile{t}{}$. %
    The main theoretical contribution of our work is provided in \cref{lemma:MFFlowW1Bound} (see \cref{appendix:EpisodicRegretBound}) which shows the following bound on the Wasserstein-1 distance between the two mean-field distributions:
    \looseness=-1
    \begin{equation*}
        W_{1} (\OptStateDist{t,h}{}, \stateDist{t,h}{}) \leq 2 \modelScale{t-1} \overline{L}_{t-1}^{h-1} \sum_{i=1}^{h-1} \int_{\stateSpace{}}
        \norm{
            \modelStd{t-1}(s, \policy{t}{}(s, \stateDist{t,i}{}), \stateDist{t,i}{})
        }_{2} \stateDist{t,i}{}(ds).
    \end{equation*}
     This shows that the deviation between the used $\OptStateDist{t,h}{}$ and $\stateDist{t,h}{}$ is bounded by the uncertainty of the statistical model integrated over $\stateDist{t,h}{}$. As the model's uncertainty decreases, the set $\mathcal{F}_{t}$ shrinks towards the true dynamics $f$ and the dynamics $\approxDynamics{}$ selected in $\cref{eq:UCBOptimization}$ is restricted to be close to $f$.
     \looseness=-1
     
     
     Next, we show an example of how the previously obtained regret bounds can be instantiated for particular models. To do so, we consider the case of Gaussian Process models.\looseness=-1
    
    \textbf{Bounds for Gaussian Process (GP) Models.}
    GP models are frequently used to model unknown dynamics in the model-based literature (see, e.g., \citet{srinivas2010gaussian, chowdhury2019online,curi2020efficient, Sessa2022EfficientComputation}). They can successfully distinguish between model's and noise uncertainty, while their expressiveness follows from different kernel functions that can be used to model different types of correlation in data.\looseness=-1
    
    Under some regularity assumptions on $f$, i.e., when the true $f$ has a bounded norm in the Reproducing Kernel Hilbert Space (RKHS) induced by the GP kernel function, these models provably satisfy
    \cref{assumption:WellCalibratedModel}. Moreover, 
    we formally show in \cref{appendix:GPRegret} that for such a GP statistical model, we can bound $I_{T}$ by the \emph{GP maximum mutual information (MMI)}. Similarly, we can express $\beta_T$ via the same quantity, and conclude that sublinearity of our regret depends on the MMI rates. \cite{srinivas2010gaussian} obtain sublinear (in the number of episodes $T$) upper bounds for this quantity in case of the most commonly-used kernels, such as the linear, squared-exponential, or Mat\'ern kernels, while \cite{Krause2011ContextualOptimization} prove sublinear bounds for certain composite kernels.
    \looseness=-1
    
    Finally, we note that the aforementioned works consider kernels defined on Euclidean spaces while our input space for $f$, namely $\jointStateSpace{} = \stateSpace{} \times \actionSpace{} \times \stateDistSpace{}$, includes the space of probability densities $\stateDistSpace{}$. Providing bounds on the GP maximum mutual information capacity in case of kernels defined on probability spaces is an interesting direction for future work.
    \looseness=-1

==> TMLR_ArXiv Submission_arXiv/sections/6-experiments.tex <==

\begin{figure*}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/initial_distribution.png}
        \caption{}
       \label{fig:initial_distribution}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/random_policy.png}
        \caption{}
        \label{fig:random_dist}
    \end{subfigure}
    \caption{\cref{fig:initial_distribution} shows the initial mean-field distribution $\stateDist{h,0}$ for each episode $h$. \cref{fig:random_dist} shows the mean-field distribution at the end of an episode using a policy that selects actions uniformly at random.}
 \label{fig:initial_distribution_random_dist}
 \vspace{-5pt}
\end{figure*}

\vspace{-1ex}
\section{Experiments}\label{section:experiments}
In this section, we demonstrate the performance of the \mfhucrl algorithm on the \textit{exploration via entropy maximization} problem introduced by \citet{Geist2021ConcaveViewpoint} and used as a benchmark problem in a recent survey on Mean-Field Games \citep{LauriereLearningSurvey}. Different from previous works, we formulate the problem in the continuous state and action spaces as follows. The state-space of the model is described by a $2$-dimensional space in $[0,11]^2$ which is split into $4$ equal-sized rooms separated by unit-sized walls with one corridor connecting neighboring rooms (See \cref{fig:initial_distribution}). Agents are free to move around within the area and are stopped by the walls if they try to move through them. Each episode $t$ consists of $21$ steps starting from $h=0$ and in each time-step $h$ the representative agent chooses its actions from the action space $\actionSpace{} = [0,1]^2$. The dynamics of the system in \cref{eq:transitionDynamics} are of the following form
\begin{equation}
\label{eq:experiment_dynamics}
    f(\state{t,h}{}, \action{t,h}{}, \stateDist{t,h}) = \state{t,h}{} +  \action{t,h}{},
\end{equation}
and the additive noise is Gaussian with zero mean, variance $\modelStd{}^2$ and independent dimensions, i.e., $\noise{t,h}{} \sim N(0, \modelStd{}^2 I_2)$ for all $t$ and $h$ where $I_2$ is the $2\times 2$ unit matrix. The individual reward function is defined as $r(\state{}{}, \action{}{}, \stateDist{}) = - \log (\stateDist{}(\state{}{}))$ meaning that the representative agent aims to avoid crowded areas. On the whole population's level, the average one-step reward is given by $\mathbb{E}_{\state{}{} \sim \stateDist{}}[-\log(\stateDist{}(\state{}{})] = - \int_{s \in \stateSpace{}} \stateDist{}(\state{}{}) \log (\stateDist{}(\state{}{}))$, so maximizing the average reward is equivalent of maximizing the population's entropy. The population is initially condensed in the bottom-left corner (as shown in \cref{fig:initial_distribution}) in a unit square, therefore, a policy is optimal if it disperses the population quickly to reach a uniform distribution.

We parameterize our policy with a Neural Network and use a Deep Ensemble model \citep{lakshminarayanan2016simple} for estimating the system dynamics. To represent the mean-field distribution, we discretize the state-space to unit squares and assign each cell the probability of the representative agent is inside of it. We provide further details on the implementation in \cref{appendix:experimentImplementation}. Additionally, we ran experiments with Gaussian Process models for the swarm motion problem to showcase the flexibility of design choices in \mfhucrl. Details and results are described in \cref{appendix:swarm_motion}.

\citet{LauriereLearningSurvey} shows that exploration is not trivial in the discrete state and action space equivalent of this environment by considering the uniform random policy which fails to reach the uniform distribution within the episode. This result holds in the continuous environment as well as shown by \cref{fig:random_dist}.

\looseness=-1

\begin{figure*}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/linear_transition_rewards.png}
        \caption{
        }
        \label{fig:results_linear_a}
    \end{subfigure}
    \vspace{1pt}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/final_dist_m3_ucrl_linear.png}
        \vspace{-5pt}
        \caption{
        }
        \label{fig:results_linear_b}
    \end{subfigure}
    \vspace{-7pt}
    \caption{Convergence of the \mfhucrl algorithm under system dynamics given by \cref{eq:experiment_dynamics}. \cref{fig:results_linear_a} shows the rewards defined in  \cref{eq:MFCOptimizationObjective} achieved by \mfhucrl over 30 episodes. Confidence bounds show the minimum and maximum over 10 independent experiments. The BPTT line corresponds to the rewards achieved under known dynamics and considered to be optimal in the environment. \cref{fig:results_linear_b} shows the close to uniform mean-field distribution at the end of the episode, $h=20$, for a policy optimised by \mfhucrl.}
 \label{fig:results_linear}
 \vspace{-5pt}
\end{figure*}
 
 \textbf{Results.} Due to the lack of an analytical solution to the problem, we compare the rewards achieved by \mfhucrl in the policy roll-outs (i.e., the interactions with the environment) to the rewards achieved by the policy optimised via the back-propagation through time (BPTT) algorithm with \emph{known} dynamics. %
We denote this policy by $\policyProfile{}{BPTT}$ and find it to be adequate since when it is used, the population's entropy quickly reaches the maximum achievable corresponding to a uniform distribution. We provide further analysis of this policy in \cref{appendix:bptt_known}.

\cref{fig:results_linear_a} shows the rewards achieved by \mfhucrl over 30 episodes. The learning can be characterized by two phases; in the first $10$ episodes \mfhucrl learns how to navigate the whole state-space, after which it reduces exploration and focuses more on fine-grained improvements. Learning to navigate the environment is challenging due to the precise movements needed to enter the corridors, especially, from an angle. Small changes in the action can decide whether the representative agent moves through the corridor to another room or is stopped by a wall. As shown by the swift improvement in \mfhucrl's performance, it successfully accumulates information in the first phase of the learning process in order to have sufficiently precise policies that can navigate the agent population through the corridors. In the second phase, it gradually refines its policy further to distribute the agents among the rooms quicker and achieve a much closer to uniform distribution as shown on \cref{fig:results_linear_b}. The optimised policy after $30$ episodes achieves a reward of $77.86$ compared to $78.26$ that of $\policyProfile{}{BPTT}$, i.e., less than $1\%$ difference.
\footnote{Animations of episodes with the BPTT policy (\texttt{known\_dynamics\_animation.mp4}) and the \mfhucrl policy (\texttt{m3\_ucrl\_animation\_episode\_t.mp4}) are included in the supplementary material. Episode $1$ to $10$ illustrate the quick learning during the exploration phase while episode $26$ is the best-performing one also used for \cref{fig:results_linear_b}.}

While \mfhucrl converges within 30 episodes, a comparable tabular Q-learning algorithm for the Mean-Field Control problem fails to achieve similar performance in more than 10 million training episodes in the discrete problem defined in \citet{Geist2021ConcaveViewpoint} and \citet{LauriereLearningSurvey}. This is most likely due to the large state space, the limitation of deterministic actions, and challenging exploration in the environment. We provide further details of the comparison and why Q-learning requires long training for convergence in \cref{appendix:comparison}.

\looseness=-1

==> TMLR_ArXiv Submission_arXiv/sections/7-conclusion.tex <==
\vspace{-1ex}
\section{Conclusion}
\label{section:Conclusion}
In this work, we propose the first model-based algorithm for the Mean-Field Control problem. The \mfhucrl algorithm runs in episodes, builds optimistic performance estimates, and uses them to efficiently explore the space during policy learning. We proved general regret bounds and showed how they can be specialized to Gaussian Process models. Furthermore, our experiments showcase the practicality of the algorithm and how it can be easily combined with deep Neural Networks. We believe that our approach provides an important step towards making model-based MARL algorithms more principled, scalable, and sample-efficient.
We see the following topics important for the further progression of the model-based mean-field learning for both the mean-field control and mean-field game problems: 1) Planning with known dynamics to solve \cref{eq:UCBOptimization} similarly to \cite{Gu2019DynamicMFCs, Motte2019Mean-fieldControls}, 2) Eliminating the need of recalibration to have Neural Networks satisfying \cref{assumption:WellCalibratedModel}, 3) Maximum mutual information bounds for kernels defined on probability spaces.
\looseness=-1


